Multiplexed Processing of Quantum Information Across an Ultra-wide Optical Bandwidth

Protocols for processing of quantum information are the foundation of quantum technology, enabling to share secrets at a distance, teleport quantum states, and to implement quantum computation. While many protocols were realized, and even commercialized, the throughput and processing speed of current protocols is limited by the narrow electronic bandwidth of standard measurement devices (typically in the MHz-to-GHz range), which is orders-of-magnitude lower than the optical bandwidth of available quantum optical sources (10-100 THz), indicating that the bandwidth resource is dramatically underutilized in current quantum optical technology. We present a general concept of frequency multiplexed quantum channels and a set of methods to process quantum information efficiently across the available optical bandwidth. Using a broadband source of squeezed light, spectral manipulation methods and parametric homodyne detection, we are able to generate, process and measure all the channels in parallel, thereby harnessing the optical bandwidth for quantum information in an efficient manner. We exemplify the concept through two basic protocols: Multiplexed Continuous-Variable Quantum Key Distribution (CV-QKD) and multiplexed continuous-variable quantum teleportation. The multiplexed QKD protocol is demonstrated in a proof-of-principle experiment, where we successfully carry out QKD over 23 uncorrelated spectral channels, with capability to detect eavesdropping in any channel. These multiplexed methods (and similar) will enable to carry out quantum processing in parallel over hundreds of channels, potentially increasing the throughput of quantum protocols by orders of magnitude.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> response_to_referees.tex <==
Reviewer 1:

The paper presents quantum processing utilizing a wide spectral band of spontaneous parametric down conversion. However, there are a lot of dubious points regarding the feasibility and/or usefulness of the scheme, as described below. Therefore, I do not think the paper is worthy for publication.

\textcolor{red}{\textbf{\textit{This is nearly rude. Especially given the misunderstanding that is later displayed. the referee is not sufficiently skilled to review the paper.}}}

 (1) In the introduction section, the paper mentions quantum computing, including trapped ions, neutral atoms, and Josephson junction. However, these items are irrelevant to this paper, and it is waste of page to mention them. Besides, it is not clear how the present scheme can be applied to quantum computing.
 \textcolor{red}{\textbf{\textit{
 1) We do not claim to present quantum computing. Quantum computing is mentioned as an application of quantum information processing to highlight the importance of the field. Moreover, the "problematic" topics (trapped ions, neutral atoms, and Josephson junction) are mentioned to give examples for quantum information processing methods as a wide glance over the existing methods. 
 
 2) We *are*  explaining how our technology can be  later applied to quantum computing (see last paragraph in the discussion section).
 
 3) We can add explanation in the introduction on how quantum teleportation is relevant for quantum computing.}}}
 
 (2) There is no description about Fig. 1 in the text, and what the paper wants to claim with Fig. 1 is not clear.
\textcolor{red}{\textbf{\textit{This is inherently wrong. The figure is referenced in the last paragraph of the intro, just before the figure itself.}}}

 (3) Characters in Fig. 1 are too small to read.
\textcolor{red}{\textbf{\textit{Accepted. Corrected}}}

 (4) Line 74 mentions that the present scheme is based on a continuous-variable analogue of the BB84 protocol using an unseeded SU(1, 1) interferometer. However, I (and maybe many readers) have not heard “SU(1, 1) interferometer.” Some references regarding this interferometer should be cited.

\textcolor{red}{\textbf{\textit{Add reference. Add a short description of SU11 as a quantum interferometer for squeezed light and entangled photons. Specifically consider SU1,1 in the weak squeezing limit of single entangled photons. Consider adding a figure, based on space availability}}}

In addition, the paper’s QKD scheme uses photon detection, which is not fit to “continuous-variable analogue,” because CV-QKD uses homodyne detection.

\textcolor{red}{\textbf{\textit{Relate to previous discussion of SU1,1 in the weak squeezing limit as a correlation detector for entangled photons}}}
 
 (5) In line 76: “broadband phase modulation device that consists of a Fourier-domain spectral shaper” is better to be reworded as “Fourier-domain spectral shaper that consists of a spatial phase modulation device.”
\textcolor{red}{\textbf{\textit{OK
}}}
 (6) Characters in Fig. 2 are too small.
\textcolor{red}{\textbf{\textit{OK}}}

 (7) The caption of Fig. 2 says that squeezed light is generated from an OPA. However, an OPA generates entangled photon pairs but not squeezed light, except at a degenerate frequency where the signal and idler frequencies are identical.
\textcolor{red}{\textbf{\textit{This is really ignorant of the referee... an OPA generates two-mode squeezed light across the entire bandwidth. In the limit of low gain this two-mode squeezed light can be described as composed of time-energy entangled photons (of a high flux).  The concept of  two-mode quadratures provides a unified framework to treat the entire bandwidth of squeezing on equal footing  (both degenerate and two-mode squeezing)
references to all our papers (initial SU11 + two-mode quadratures}}}
 
 (8) The present protocol encodes data by a spatial modulator, whose modulation speed is slow compared with a phase modulator used in optical communication. Subsequently, it is suspicious if the paper’s QKD scheme achieve a high key-creation rate in terms of bits per seconds, even though the number of QKD channels is increased with frequency division multiplexing.
\textcolor{red}{\textbf{\textit{This is being picky on technical details. We never claimed high speed ! This is a mere proof-of-concept. However, the speed of the single-channel is  fundamentally limited only by the channel bandwidth. The speed of the phase modulator is only a technical limit that can be lifted in many possible ways. Let us mention only two of them. First, using fast acusto-optic modulators as the phase modulators that can easily reach update-rates at the MHz scale. And second, one can remove the need to modulate altogether by resorting to an entanglement-based protocol (a multiplexed version of Eckert 91)}}}
 
 (9) In line 80: a pump laser is assumed to pass through two OPAs in series. However, the pump wavelengths in $2\omega$-based OPA is 0.75 $\mu$m, at which the fiber attenuation is large. Subsequently, the pump light at the 2nd OPA is weak, and it is suspicious if the paper’s scheme is feasible for QKD over fiber transmission lines.
 \textcolor{red}{\textbf{\textit{This is again picking on a technical point. Indeed 780nm will not pass easily through long fibers, but it just doesn't need to. remember that the pump is classical and can therefore be easily regenerated locally from an appropriate local oscillator that is shared between the parties. For example, one can use the degenerate frequency at 1560 as that LO (which is very-well transmitted through the fiber)}}}

 (10) In the present QKD protocol, the SPDCs generated in the 1st and 2nd OPAs interfere with each other. However, the relative phases between signal, idler, and pump lights change through fiber transmission due to the chromatic dispersion. In addition, the relative polarization states between them also change due to the fiber birefringence. Subsequently, it is suspicious if a designed interference occurs.
\textcolor{red}{\textbf{\textit{Another technical annoyance... Indeed dispersion affects the phases of the frequency pairs, but dispersion is just a deterministic quadratic-phase modulation across the spectrum that can easily be compensated by a wide-variety of means for any amount of dispersion. Weak dispersion can be easily compensated directly by the phase modulator (different phase reference for every channel) and larger values of dispersion can be mitigated with dispersion-compensating fibers of the appropriate length. }}}
 (11) In line 107, the parametric gain g should include the pump light amplitude and phase, which are different in the 1st and 2nd OPAs, as mentioned above.
 \textcolor{red}{\textbf{\textit{add the phase to the line to keep him quiet...}}}

 (12) In the 2nd OPA, the signal and idler lights coming from the 1st OPA are amplified as well as SPDC is generated. I wonder if a proper interference occurs under such condition.
\textcolor{red}{\textbf{\textit{This is a critical misunderstanding on behalf of the referee, since the amplification is not separate from the inteterference - they are one and the same!. Specifically, the OPA is a phase-dependent amplifier that can either amplify (stretch) or deamplify (squeeze) the incoming light dempending on the phase of the signal-idler pair relative to the pump.}}}
 
 (13) I am afraid that the abovementioned amplification is not considered in Eq. (1).
\textcolor{red}{\textbf{\textit{it is. see above}}}

 (14) In Bob’s detection, the mean photon number incident to a detector is much less than one in a QKD system, and the detection efficiency is also less than one. Subsequently, it is suspicious if destructive interference and no-photon event can be distinguished.
 \textcolor{red}{\textbf{\textit{Indeed, the no-photon event and destructive interference result both in 0 photons in the detectors meaning that they cannot be distinguished during the measurement, however the probability for no photons is still dependent on Alice's phase resulting in a noisy channel which still can transfer information. The amount  of information (as we will show in a future paper) is simply calculated using the definition of channel capacity from information theory and is definitely greater than zero meaning that Alice and Bob can communicate over such a channel.}}}

 (15) The mean photon number per channel should be less than one for the security, and, to guarantee this condition, the number of signal-idler pair should be less than one over the whole spectral range. Subsequently, it is suspicious if a high key-creation rate in terms of bits per second can be achieved, even though frequency-division multiplexing is employed.
 \textcolor{red}{\textbf{\textit{False! Only the average number of photons per channel should be less than 1 but the total number of photons across the spectrum is not limited at all, and can be much larger than one.}}}


 (16) In Section 2, quantum mechanical operators should be attached with a hat.
 \textbf{\textit{OK. We'll add a hat}}

 (17) The theoretical analysis in the second last paragraph in Section 2 misses the generation of multiple pairs that can cause bit errors because the signal/idler phases of pairs A and B are different.
 \textbf{\textit{No. Multiple pairs in a single channel  will not have different phases. Indeed, the phase of each photon (frequency) is random, but the phase-sum of  the signal-idler pair is fixed by the pump (and propagation). Thus, no phase ambiguity will arise, even if multiple photons are emitted}}

 (18) In the last paragraph in the last paragraph in Section 2, a beam splitting attack is detected from the photon number reduction resulting from the beam splitting. In the QKD study, however, Eve is assumed to use a lossless transmission line for not changing the photon number at Bob. The paper’s consideration is against the standard assumption in the QKD field.
\textbf{\textit{To detect Eve, we do not rely on the average intensity, but rather on the interference contrast. Specifically, on how destructive is the dark fringe. Eve's presence will inevitably reduce the contrast as we discuss. 
If Eve tries to cover her tracks by injecting entangled photons of the same pump with a random phase she will introduce even more errors that Alice and Bob can easily detect (Add this calculation to the supplementary)}}

 (19) Characters in Fig. 3 are too small to read.
\textbf{\textit{OK}}

 (20) Section 3 presents multiplexed quantum teleportation utilizing broadband squeezed lights. However, squeezed light is generated at a degenerate frequency at which the signal and idler frequencies are identical. Subsequently, it is suspicious if broadband squeezed light can be generated.
\textbf{\textit{Same mistake as before. Squeezed light is generated across the spectrum and at a single frequency}}

 (21) Squeezed light cannot be transmitted because it is fragile against attenuation. Then, I wonder what is an application of the present quantum teleportation scheme. Although, the manuscript indicates quantum computing, it is desired to specify how beneficial when the present scheme is applied to quantum computing.
\textbf{\textit{We need to add a paragraph of measurement-based computing with cluster states, as we stated before}}


 (22) The loss effect should be considered in Eq. (5) for practical applications.
\textit{\textbf{OK. We'll add it}}
%%%%%%%%%%%%%%%%%%%%%%%%
 (23) The experiment in Section 5 uses intense light, which cannot be regarded as a QKD system. Weak coherent light and single-photon detectors should be used to claim that a QKD scheme is experimentally demonstrated.
\textbf{\textit{We don't use strong light. Our intensity is weak with  less than 1 photon /$\mu s$ /channel @@@verify@@.  We choose long integration times in order to simply reconstruct the photon probabilities of the different channels.@@@need to improve the argument - maybe claim that the interference is the quantum coincidence detector@@@ }} 

\textit{\textbf{In our experiment: 10000 / ms / channel
Channel bandwidth > 100GHz
Quantum state coherence time < 10ps
Avg. photons per quantum state = 10000 * 1000 / 10^11 = 10^4 * 10 ^ 3 / 10 ^11 = 10^-4}}

  Reviewer \#2

The paper “Multiplexed Processing of Quantum Information Across an Ultra-wide Optical Bandwidth” by ELDAN et al. presented a general concept and methods to process quantum information in parallel over multiplexed frequency channels by exploiting a phase sensitive parametric amplifier to serve as homodyne detection for measurement of all the channels simultaneously. Based on basic structure of SU(1,1) interferometer, the authors proposed two basic protocols : multiplexed QKD and multiplexed quantum teleportation. The former/latter is for SU (1,1) in low/high gain regime. Additionally, the authors demonstrated a proof-of principle experiment about multiplexed QKD. I think the ideal is interesting. However, I do not paper meets the standard of Optica. The main reasons are the following: 

1) The key of the proposed protocols is to realize the homodyne detection by using phase sensitive optical parametric amplifier (PSOPA) in combination of an array of power detectors. In fact, following the pioneer work reported in Ref. [24] (Nat. Commun. 9, 609 (2018)), this detection method had been in-depth studied by a few other groups from both the theoretical and experimental aspects (OE, 27, 30552 (2019), Phys. Rev. A, 101, 053801 (2020), OE, 28, 34916(2020), and Applied Physics Letters 122, 104001 (2023)…). I agree that the parametric homodyne detection realized by the combination of high gain PSOPA and an array of power detectors can be used to measure the optical quadrature across a wide band. However, comparing with the traditional homodyne detection (HD) widely used in CV quantum information, the parametric homodyne detection method has some shortcomings. For example, in the sense that HD measurement can amplify the quadrature amplitude of probe, the gain of PSOPA is equivalent to power of strong local oscillator of traditional HD. However, comparing with amplification provided by the strong local oscillator, the amplification of provided by the gain of PSOPA is quite low. Therefore, I think the protocols proposed in this paper will be misleading unless a detailed analysis about the suitable application range of this parametric homodyne detection method is provided 

\textbf{\textit{In short - we don't really need to measure the quadrature amplitudes. All we need is SU1,1 interference with a high contrast. Note that for $g_1=g_2$, the contrast of SU1,1 is 100\% always, independent of the gain . This is the only feature of SU1,1 we employ, both at the low gain regime (for QKD) and at the high gain regime (for teleportation). 

Our description was too loose, and a bit negligent in naming our measurement "parametric homodyne". Indeed, to measure a single quadrature with parametric homodyne, the gain for the measurement  OPA must be very high, but this is not necessary for our scheme to work.

@@@We need to carefully reword  our text to reflect this. Think of how and where...}}

2) For traditional HD, the information encoded on quadratures X and Y can be flexibly extracted out by varying the phase of local oscillator. I wonder if the parametric homodyne detection realized by the combination of phase sensitive optical parametric amplifier (PSOPA) and power detectors has the ability to simultaneously decode the information encoded on quadrature amplitudes X and Y? Moreover, in practice, the application of broadband squeezed light with 10-100THz of bandwidth should consider the dispersion effect. We know that the PSOPA used to measure squeezing should be operated at de-amplification condition. When the dispersion induced phase shift starts to play a role, how can we manage the PSOPA to ensure it running at de-amplification condition across the broad band of 10-100 THz? 

\textbf{\textit{Since $[x,y]>0$, the quadratures  $x$,$y$ cannot be measured simultaneously. Thus, parametric homodyne cannot measure both quadratures (just like in standard homodyne). Note that at no point does our protocol require (or our experiment measure) both quadratures. Each parametric measurement relates to a single quadrtature only.

Moreover, to encode our quantum information in the protocols we rely on the quadrature-bases being mutually unbiased, just like in standard BB84.

As for the dispersion, it is easy to take into accout and compensate, see response to referee #1 above}}

3) One important point that has not been considered is the influence of path length difference between difference channels upon the detection. For multiplexed information processing, different channels usually carried different information and propagates through different optical path. As a result, the optical path length in different frequency channel will be quite different, and the path length difference between the channels of signal and idler photon pairs may exceed the coherence length [see the papers “Quantum optical coherence: From linear to nonlinear interferometers” (Phys. Rev. A 104, 043707 (2021)) and “Temporal coherence in an unbalanced SU(1,1) interferometer” ( Opt. Lett. 48, 127 (2023)) for details). When the path length difference of signal and idler fields is greater than coherence of individual signal/idler filed (depends on the frequency bandwidth of the channels), the second optical parametric amplifier in Figs 1-3 will become phase insensitive, no interference can be observed at the output port. As a result, the proposed protocols may fail. 

\textbf{\textit{When considering coherence lengths, we should note the stark difference between the single-photon coherence time, which reflects the stability of the single phases $\varphi_{s,i}$ independently and is indeed inversely proportional to the channel bandwidth; and the two-photon coherence time, which reflects the stability of the phase sum $\varphi_s+\varphi_i$ relative to the pump and is dictated only by the pump coherence time, which is very long  (the pump is spectrally very narrow, <50KHz in our experiment), far longer than  delay that may arise experimentally. In our SU1,1, we worry only about the latter, so delay is not a problem. 

Furthermore, note that the parametric amplification operates on the entire bandwidth of all frequency channels simultaneously BEFORE we  separate the different channels to be measured. Thus, the only path difference that matters is the one accumulated between the parametric amplifiers due to chromatic dispersion during propagation. As mentioned before, we compensate for the dispersion either by a dispersion compensating medium of appropriate length or by the phase modulation and calibration in the spectral shaper (the SLM in the experiment). }}

4) The concept of parametric homodyne detection is not clearly defined. Traditional HD usually requires the satisfaction of the condition：the intensity of LO is much greater than that of probe field. I agree that a high gain PSOPA followed by a power detector is equivalent to a traditional HD. However, in this paper, the detection realized by the OPAs running at low gain regime is also referred to as homodyne detection. When the two optical parametric amplifiers (OPAs) are running at low gain regime, the detection is based the interference between the photon pairs generated from the two OPAs with same gain. In this case, is the name “homodyne detection” still appropriate? 

\textbf{\textit{Correct. This indeed requires a semantic clarification. See response above}}

5) I am not convinced by the experimental results. The authors say “a bare interference contrast of 75\%” and “the initial loss in our simple configuration was relatively high ( 44\%)”, and more detailed experimental results are given in Fig. 2 (in Supplemental document), in which the data points will fit the theory curve given by Eq. (4). The reason that I am not convinced by experimental results are three folds. First, the curve representing the theory expectation can be obtained by substituting the value loss into Eq. (4). The calculated value should be V=61\% for T=44\%, but not 75\%. Second, I do not think that the experimental results can be analyzed by directly using Eq. (4). Because Eq. (4) is obtained by assuming the gains of two OPAs are the same, however, the gains of two OPAs in the experiment should be different. The pump power of second OPA will be definitely lower than that of first OPA. When the residual pump of first OPA is reflected and coupled into PPLN, significant loss will be introduced. With the loss of pump for second OPA considered, the theoretically expected value of visibility will be further decreased (please see the paper “Lossy SU(1,1) interferometers in the single-photon-pair regime” [DOI 10.1088/2058-9565/acc205] for details). 
\textbf{\textit{Referee may have missed a point. In our experiment, the measured LOSS was 0.44, while referee calculated the contrast assuming TRANSMISSION of 0.44. When we substitute T=1-0.44=0.56 the constrast becomes \~ 0.72 which is much closer to our measured contrast (0.75). The remaining difference may be a result of a slight misalignment in the setup between different measurements.}}

\textbf{\textit{Pump loss is irrelevant. The pump is a classical field that can be easily amplified at will with no consequences. Specifically in our experiemtn we used pump replacement and we did make sure that the two parametric gains were equal. We thank the referee for the point about "lossy SU1,1", which may be used in the future to expand the validity of our model also to lossy situations, but it is beyond the scope of our discussion here.}}

Minor points: 

(1) We know BB84 scheme belongs to discrete variables. Since the encoding and decoding of the proposed QKD scheme are similar with that of BB84, I wonder why the authors claim they proposed CV-QKD protocol. 

\textbf{\textit{Accepted. We should change the presentation to tone down the CV aspects (and those of PHD).}}

(2) From the protocols in Figs 1-2, one sees that the stage of channel manipulation stage is in between two optical parametric amplifiers, which will inevitably introduce loss and lead to a degradation of quantum advantage no matter what kind of measurement method is exploited. When the light carrying information is coupled into second OPA for measurement, there exit extra loss (comparing with the traditional HD), which will further degrade the quantum advantage. So I wonder if the proposed protocol is practically useful. 

\textit{\textbf{The loss is not greater than standard HD. The shaper loss can be very low, The OPA coupling loss is equivalent to mode-matching loss in standard HD, and is of the same order of magnitude. If at all, SU1,1 has an advantage over standard HD since it is insensitive to detector-inefficiency as opposed to HD, which interprets detector inefficiency also as loss. }}

(3) The font in Figs. 1-3 is too small to read. 
\textbf{\textit{OK}}

(4) There are typos. (i) page 3, 7th line, “her”;…
\textbf{\textit{OK}}

